NeO 360: Neural Fields for Sparse View Synthesis of Outdoor Scenes

Recent implicit neural representations have shown great results for novel view synthesis. However, existing methods require expensive per-scene optimization from many views hence limiting their application to real-world unbounded urban settings where the objects of interest or backgrounds are observed from very few views. To mitigate this challenge, we introduce a new approach called NeO 360, Neural fields for sparse view synthesis of outdoor scenes. NeO 360 is a generalizable method that reconstructs 360{\deg} scenes from a single or a few posed RGB images. The essence of our approach is in capturing the distribution of complex real-world outdoor 3D scenes and using a hybrid image-conditional triplanar representation that can be queried from any world point. Our representation combines the best of both voxel-based and bird's-eye-view (BEV) representations and is more effective and expressive than each. NeO 360's representation allows us to learn from a large collection of unbounded 3D scenes while offering generalizability to new views and novel scenes from as few as a single image during inference. We demonstrate our approach on the proposed challenging 360{\deg} unbounded dataset, called NeRDS 360, and show that NeO 360 outperforms state-of-the-art generalizable methods for novel view synthesis while also offering editing and composition capabilities. Project page: https://zubair-irshad.github.io/projects/neo360.html

==> iccv2023AuthorKit/sections/13_additional_quanitative_results.tex <==

\section{Additional Quantitative Results:}
\label{sec:add_quantitative_results}

\input{iccv2023AuthorKit/tables/additional_comparisons}

We include additional baseline comparisons with overfitting NeRF baselines~(mipNeRF360~\cite{barron2022mip} and EG3D~\cite{chan2022efficient}) and generalizable NeRF baseline~(SRT~\cite{srt22}). We include these comparisons in Tab.~\ref{tab:add_comparison}. One could clearly observe that naively using triplanes~(Tab.~\ref{tab:add_comparison} row 3, *denotes that we take the triplanar representation without generative losses or training) or local features as in PixelNeRF~(our paper Tab.~\textcolor{red}{4})  hurt the performance. Our method relies on effective combination of local and global features which serves as a strong baseline for the challenging task of 360$^{\circ}$ view synthesis of outdoor scenes. This is further confirmed by our superior results against added baselines~(Tab.~\ref{tab:add_comparison}) and qualitative results~(cf. supp. video). We also include depth reconstruction metrics~(Tab.~\ref{tab:depth_metrics}) and show our techniques' superior results compared to Pixel-NeRF.

\textbf{Difference from~\textit{EG3D} and~\textit{GAUDI}:} Both approaches are generative models which use adversarial losses for training and GAUDI uses GAN inversion for conditional synthesis. Our approach, NeO 360, does not rely on expensive GAN inversion and directly outputs density/RGB for all test views. Motivated by your excellent comments, we add a baseline~(Tab.~\ref{tab:add_comparison} row 3) comparing EG3D/GAUDI's representation i.e. triplanes which reduces to a vanilla NeRF variant optimized per scene. We leave the generative counterpart comparisons to future work and hope our dataset is a useful to the community in that direction.

==> iccv2023AuthorKit/tables/depth_metrics.tex <==
\setlength{\columnsep}{6pt}%
\begin{wraptable}{r}{0pt}
\scriptsize
\centering

\begin{tabular}{@{}lcc@{}}
\toprule
Object Depth & \textbf{L1} ↓ & \textbf{RMSE} ↓  \\ 
\midrule
PixelNeRF~\cite{yu2021pixelnerf} & 0.83 & 1.07  \\
NeRO~(no ft.) & 0.59 & 0.74\\
\midrule
~\textbf{NeRO~(Ours)}   & \textbf{0.20} & \textbf{0.61}\\
\bottomrule
\end{tabular}

\caption{Eval views depth prediction from 3 source views on NeRDS360}
\vspace{-3pt}
\label{tab:depth_metrics}

\end{wraptable}
